Learning Likely Invariants to Explain Why a Program Fails

Debugging is difficult. Recent studies show that automatic bug localization techniques have limited usefulness. One of the reasons is that programmers typically have to understand why the program fails before fixing it. In this work, we aim to help programmers understand a bug by automatically generating likely invariants which are violated in the failed tests. Given a program with an initial assertion and at least one test case failing the assertion, we first generate random test cases, identify potential bug locations through bug localization, and then generate program state mutation based on active learning techniques to identify a predicate "explaining" the cause of the bug. The predicate is a classifier for the passed test cases and failed test cases. Our main contribution is the application of invariant learning for bug explanation, as well as a novel approach to overcome the problem of lack of test cases in practice. We apply our method to real-world bugs and show the generated invariants are often correlated to the actual bug fixes.

==> conclusion.tex <==
\section{Discussion} \label{conclusion}


==> discussion.tex <==

\section{Discussions}
We explain the limitations associated with our hybrid approach for predicate abstraction in this section.
\subsection*{False Positive Transitions}
During verification of the NFA, false positive transitions may be added by symbolic execution. For example when trying to prove the $push$ transitions leaving state $\bar{p}\bar{q}$ in Figure~\ref{nfa_1}, there is only one feasible transition which goes to state $p\bar{q}$. The union of postconditions of these transitions is the formula $p\bar{q}$. So the verification condition in proving the $push$ on state $\bar{p}\bar{q}$ is $(size < 1\wedge size < 5)\wedge SymbExeTree(push)\Rightarrow(size \geq 1 \wedge size<5)$. Symbolic execution engine finds that this verification condition is not valid as evidenced by the counterexample assignment: $size = -1$, from this assignment we can infer that the transition $\bar{p}\bar{q}\xrightarrow{push}\bar{p}\bar{q}$ is feasible. But the assignment is false positive as $size$ cannot be negative. The concrete execution of push under this counter example input will cause out of bound error when accessing the array field $data$. The false positive is caused by the underlying symbolic execution engine's incapability to handle arrays. When accessing the array field $data$, SPF does not add array bounds checking conditions to the path formula to make sure that the array access under the concrete input is not out of bounds. Thus we need to make assumption about the capacities of underlying symbolic execution engines.

\subsection{Granularity of Abstraction}
Our approach currently is only able to compute the predicate abstraction at the function level while traditional predicate abstraction techniques compute the abstraction for each statement in the method. The granularity does matter for concurrent programs where the level of atomicity does influence the results.

\subsection{Problems with Alphabet Refinement}
It is possible that during membership queries there is no predicate able to distinguish the inputs of an inconsistency sequence of method calls. This is related to the inadequacy of the set of given predicates. For example, in the \textit{BankAccount} example, the given set of predicates for the class is $balance \geq 1$ and the set of predicates given for method \textit{deposit($amount$)} is $amount \geq 1$. There is no predicate which is able to distinguish the sequence $\langle deposit, deposit\rangle$ with two concrete test cases $\langle deposit(-10), deposit(10)\rangle$ and $\langle deposit(-1), deposit(8)\rangle$. This problem is deeply related to the inherent non-determinism in predicate abstraction and the limitation of $L^*$ algorithm that it is only able to learn DFA. NFA is much better than DFA for modeling systems with non-determinism~\cite{cdnf:CAV2010} as the number of states of the NFA is exponentially smaller than that of an equivalent DFA. Is there any variant of $L^*$ algorithm or any other learning algorithm to learn an NFA? Perhaps, we can use the family of CDNF algorithms~\cite{cdnf:IC1995,cdnf:CAV2010,bull:CAV2013} to learn a Boolean formula.

We cannot use the Residual NFA learning algorithm~\cite{nlstar:IJCAI2009} to learn an NFA as its assumption requires the answer of membership query to be either ``yes'' (\verb"true") or ``no'' (\verb"false") but not both and it uses the ``union'' operator (the logic or operator ``$\vee$'') to find composite rows in order to reduce the number of states in the final NFA. In essence it can only learn an equivalent NFA (with smaller number of states) of a DFA.

\subsection{The Wishful Thinking Problem}
We need to store for each guard the passing parameter values, otherwise the learning algorithm will not converge.

\subsection{Failed Concrete Execution with SPF Returned Values}
When the execution of target method with returned concrete values fails, we can weaken the precondition by remove the passing method predicates and prove again.
\subsection{Optimizations} 

==> preliminary.tex <==
\section{Preliminaries} \label{pre}
In the following, we formally define our problem on abstracting a Java class.

%In this section we introduce some preliminaries about mealy machine, active learning algorithm for mealy machine and predicate abstraction, all of which are used in our hybrid predicate abstraction approach.

\subsection{The Problem}
Without loss of generality, we assume a Java class $\cal C$ contains a finite set of class variables $X$ and a finite set of methods $M$, each of which potentially updates variables in $X$. The semantics of $\cal C$ is a labeled transition system $(S_c, s_c, M, T_c)$ where $S_c$ is a set of states, each of which is a valuation of all variables in $X$; $s_c \in S_c$ is the initial state; and $T_c: S_c \times M \times S_c$ is the smallest transition relation such that $(s, m, s') \in T_c$ if and only if, given the variable valuation $s$, executing method $m$ results in variable valuation $s'$.

Our problem is to construct an abstraction of $\cal C$ automatically. Let $Prop$ be a set of propositions constituted by variables in $X$. We write $2^{Prop}$ to denote the set of predicates which can be formed by conjuncting a subset of propositions in $Prop$ and the negation of the rest of the propositions. We write $s \models \phi$ to denote that $\phi$ evaluates to true given the variable valuation $s$. An abstraction of $\cal C$ with respect to $Prop$, denoted as $\cal A$, is a labeled transition system $(S_a, s_a, M, T_a)$ where $S_a \subseteq 2^{Prop}$ is a set of abstract states; $s_a \in S_a$ satisfies $s_0 \models s_a$; $T_a \subseteq S_a \times M \times S_a$ is the smallest transition relation such that $(\phi, m, \phi') \in T_a$ if and only if there exists $(s, m, s') \in T_c$ such that $s \models \phi$ and $s' \models \phi'$. A naive approach to construct $\cal A$ would be to check whether every possible transition$(\phi, mt, \phi')$ where $\{\phi, \phi'\} \subseteq S_a$ and $mt \in M$ is contained in $\cal A$. This is perhaps infeasible since by definition, there could be, in the worse case, $2^{\#Prop} * \#M * 2^{\#Prop}$ number of transitions in $\cal A$ where $\#Prop$ is the number of the propositions and $\#M$ is the number of methods. Thus, we propose to learn the abstraction, based on testing instead, through an intermediate model in the form of a Mealy machine.

\subsection{Mealy Machine}
Mealy machines~\cite{mealy:BLTJ1955} were originally proposed to model the behavior of reactive systems with inputs and outputs. A Mealy machine $\cal{M}$ is defined as a tuple $\langle Q, q_0, I, O, \delta \rangle$, where $Q$ is a finite set of states; $q_0 \in Q$ is the initial state; $I$ is a finite set of input symbols; $O$ is a finite set of output symbols; $\delta: Q \times (I \times O) \times Q$ is a labeled transition relation. A transition is often denoted as $(q, i/o, q')$, which intuitively reads: as state $q$, with input $i$, the system outputs $o$ and transits to state $q'$. In this work, we use Mealy machines as an intermediate model for behavior of the given class. The input symbol set $I$ is defined as $2^{Prop} \times M$ and the output symbol set $O$ is defined as $2^{Prop} \cup \{\bot\}$. For instance, a transition $(q, (size \geq 0, push)/(size \geq 0), q')$ intuitively means that at state $q$, invoking $push$ when the predicate $size \geq 0$ may result in a variable valuation satisfying $size \geq 0$ and lead to state $q'$. The special output $\bot$ denotes that the result is an exception. A trace of $\cal{M}$ is a sequence of input/output pairs which can be generated traversing through the states of the machine.
    
%An unknown transition $s\xrightarrow{g.m/\top}\top$, represents executing $m$ on state $s$ which does not satisfy the guard condition $g$. Unknown transition happens due to the limited coverage of parameters generated by random testing. An input trace $tr=\langle g_0\cdot m_0, g_1\cdot m_1,\cdots,g_k\cdot m_k\rangle$ represents a sequence of method calls to $m_0,m_1,\cdots,m_k$ with satisfying transitions $s_i\xrightarrow{g_i\cdot m_i/g_{i+1}}s_{i+1}$ for all $0\leq i < k$ and $s_0=q_0$.

One of the reasons that we adopt Mealy machine as an intermediate representation is that there is an effective learning algorithm ${L_M}^+$ Algorithm~\cite{lmstar:FM2009} for learning Mealy machines. Let $\mathcal{M_U}$ be an unknown Mealy machine which is to be learned. ${L_M}^+$ learns a Mealy machine $\mathcal{M_U}$ from a teacher who knows $\mathcal{M_U}$, by asking a series of membership queries and candidate queries. A member query asks whether a sequence of input/output pairs is a trace of $\mathcal{M_U}$. The teacher answers the queries based his/her knowledge of $\mathcal{M_U}$. For instance, the teachers answers yes iff it is a trace of $\mathcal{M_U}$. For instance, in the Stack example, a membership query would be: $\langle (size \geq 0, push)/(size \geq 0), (size \geq 0, pop)/(size < 0) \rangle$, which asks whether or not it is true that invoking $push$ when $size \geq 0$ would result in a state satisfying $size >0$ and then $pop$ would result in a state satisfying $size < 0$. After multiple membership queries, the ${L_M}^+$ algorithms forms a guess what the Mealy machine by \emph{generalization} what it has learned so far and asks a candidate query. A candidate query asks whether a candidate Mealy machine is equivalent to $\mathcal{M_U}$. If the answer to a candidate query is negative, the teacher provides a counterexample in the form of a sequence of input/output pairs. ${L_M}^+$ then asks another series of membership queries and another candidate query until the answer to the candidate query is yes, in which case, the Mealy machine has been learned successfully. The complexity of the ${L_M}^+$ algorithm is $O(|I|^2n + |I|mn^2)$, where $|I|$ is size of input alphabet, $n$ is number of states in the minimum Mealy machine and $m$ is maximum length of counterexamples.

%\subsection{Predicate Abstraction}

%Given a set of predicates $P=\{p_1, p_2,\cdots, p_n\}$, a predicate abstraction for formula $\psi$ w.r.t. $P$, denoted as $G_P(\psi)$, is defined as the strongest postcondition implied by $\psi$, i.e., $\psi \models G_P(\psi)$, in which all the atomic predicates are from $P$. A $minterm$ of $P$ is defined as $p_{1}^{k_1}\wedge _{2}^{k_2}\wedge \cdots\wedge p_{n}^{k_n}$ in which every $k_i\in\{0,1\}$ and $p_{i}^{0}={\bar{p_i}}, p_{i}^{1}=p_i$. Then $G_P(\psi)$ is also defined as \[G_P(\psi)=\vee\{\phi| \phi \text{ is a minterm of } P \text{ and } \phi\wedge\psi \text{ is satisfiable}\}\] thus we are doing the Boolean Abstraction~\cite{cartesianAbs:TACAS2001} instead of the more coarse but more efficient Cartesian Abstraction~\cite{cartesianAbs:TACAS2001}. All existing approaches for predicate abstraction are purely using SMT solvers to check the satisfiability of $\phi\wedge\psi$ for each minterm $\phi$. The cost of these approaches is that there are $2^n$ minterms which need to be checked in the worst case.

%Given the above definitions, we can learn a partial Boolean abstraction of each method defined in the target Java class in a naive way by enumerating all the minterms of the given set of predicates and concatenate with each method to form the input alphabet and use all the minterms and the $error$ to form the output alphabet for the mealy machine learner. The problem with this approach is that there are $2^n$ minterms, thus the learning algorithm is intractable.



